DeFi versus TradFi: Valuation Using Multiples and Discounted Cash Flows

As of August 2022, blockchain-based assets boast a combined market capitalisation exceeding one trillion USD, among which the most prominent are the decentralised autonomous organisation (DAO) tokens associated with decentralised finance (DeFi) protocols. In this work, we seek to value DeFi tokens using the canonical multiples and discount cash flow (DCF) approaches. We examine a subset of DeFi services including decentralised exchanges (DEXs), protocol for loanable funds (PLFs), and yield aggregators. We apply the same analysis to some publicly traded firms and compare them with DeFi tokens of the analogous category. Interestingly, despite the crypto bear market lasting for more than one year as of August 2022, both approaches evidence overvaluation in DeFi.

==> tables/comparables.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} & \multicolumn{2}{l}{Market Data} & Financial Data & \multicolumn{2}{l}{Estimations} \\
{} &        Prices &       Mkt Cap &            TVL &       Mkt Cap & Protocol Revenue \\
token &               &               &                &               &                  \\
\midrule
IDLE  &      2.037693 &  5.436950e+06 &   1.038275e+08 &  2.076550e+07 &     2.076550e+06 \\
COMP  &    200.170816 &  1.266899e+09 &   8.923174e+09 &  1.784635e+09 &     1.784635e+08 \\
UNI   &     17.058302 &  7.753293e+09 &   8.414520e+09 &  1.682904e+09 &     1.682904e+08 \\
BAL   &     17.534129 &  1.895901e+08 &   3.285260e+09 &  6.570519e+08 &     6.570519e+07 \\
AAVE  &    255.543328 &  3.459438e+09 &   1.434394e+10 &  2.868788e+09 &     2.868788e+08 \\
YFI   &  33025.884788 &  1.188961e+09 &   4.120927e+09 &  8.241853e+08 &     8.241853e+07 \\
\bottomrule
\end{tabular}

